Reasoning-Guided Grounding: Elevating Video Anomaly Detection through Multimodal Large Language Models

Video Anomaly Detection (VAD) has traditionally been framed as binary classification or outlier detection, providing neither interpretable reasoning nor precise spatial localization of anomalous events. While Vision-Language Models (VLMs) offer rich scene understanding, they struggle with reliable spatial grounding - often producing hallucinated or geometrically invalid bounding boxes when asked to localize objects. We propose VANGUARD (Video Anomaly Understanding through Reasoning and Grounding), a framework that unifies anomaly classification, spatial grounding, and chain-of-thought reasoning within a single VLM. VANGUARD introduces a three-stage curriculum that progressively layers training objectives: (1) classifier warmup on frozen backbone features, (2) LoRA-adapted spatial grounding, and (3) chain-of-thought generation. To overcome the sparse annotation typical of VAD benchmarks, we employ a teacher-student annotation pipeline in which a VLM (Qwen3-VL-4B) generates structured per-subclip reasoning trajectories based on manual annotations available from the UCA Dataset. Further, GroundingDINO provides bounding box supervision. On UCF-Crime, VANGUARD achieves 94% ROC-AUC with 84% F1 while simultaneously producing interpretable chain-of-thought explanations and spatial grounding of anomalous objects - capabilities absent from prior VAD methods. Ablations confirm that staged training outperforms monolithic optimization, and that structured reasoning acts as an implicit regularizer yielding more balanced predictions than classification-only fine-tuning. Zero-shot transfer to XD-Violence and ShanghaiTech demonstrates cross-domain generalization without target-domain adaptation.

==> sections/impact.tex <==
% Impact Statement Section (Supplementary)
\section{Impact Statement}
\label{app:impact}

This work on video anomaly detection with spatial grounding has direct applications to surveillance systems, carrying both benefits and risks. On the positive side, interpretable anomaly detection can improve response times, reduce false alarms, lower the cognitive burden on human monitors, and---unlike black-box systems---produce auditable natural language explanations. However, video surveillance inherently raises privacy concerns, and deployment should occur only with appropriate legal authorization and data protection measures. Our teacher-student pipeline inherits biases from GroundingDINO and Qwen3-VL, and UCF-Crime's predominantly US footage means the model's notion of ``anomalous'' behavior reflects a specific cultural context; thorough bias auditing is essential before deployment. As with any computer vision technology, misuse for authoritarian surveillance is possible, and generated explanations should support rather than replace human decision-making. Throughout this research, we used only publicly available datasets, designed the system for human oversight, and will release code with clear usage guidelines. We believe the interpretability advances in this work can improve responsible deployment of video monitoring systems, but urge practitioners to implement appropriate safeguards and prioritize human rights in any surveillance application.

